Motivations, Challenges, Best Practices, and Benefits for Bots and Conversational Agents in Software Engineering: A Multivocal Literature Review

Bots are software systems designed to support users by automating a specific process, task, or activity. When such systems implement a conversational component to interact with the users, they are also known as conversational agents. Bots, particularly in their conversation-oriented version and AI-powered, have seen their adoption increase over time for software development and engineering purposes. Despite their exciting potential, ulteriorly enhanced by the advent of Generative AI and Large Language Models, bots still need to be improved to develop and integrate into the development cycle since practitioners report that bots add additional challenges that may worsen rather than improve. In this work, we aim to provide a taxonomy for characterizing bots, as well as a series of challenges for their adoption for Software Engineering associated with potential mitigation strategies. To reach our objectives, we conducted a multivocal literature review, reviewing both research and practitioner's literature. Through such an approach, we hope to contribute to both researchers and practitioners by providing first, a series of future research routes to follow, second, a list of strategies to adopt for improving the use of bots for software engineering purposes, and third, enforce a technology and knowledge transfer from the research field to the practitioners one, that is one of the primary goal of multivocal literature reviews.

==> old/rq_1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{RQ\textsubscript{1}: On the use of bots and conversational agents for software engineering purposes}
%\filomena{è epressa diversamente precedentemente}
%\topar{obiettivo della domanda di ricerca}
As a first goal, we aimed to identify the motivations and objectives behind the adoption of bots for software engineering purposes. Our purpose was to gather general and fundamental pieces of information to (1) define a taxonomy to categorize bots based on their use and (2) better perform the following research step.

%\topar{come si sono riportati i risultati?}
For readability reasons, we categorize the bots under three main categories--subsequently divided into sub-categories---depicted in Figure \ref{fig:motivations}. We relied on the narrative synthesis and thematic analysis techniques to extract such categories—the process has been detailed in Section \ref{sec:methodology}.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/motivation.pdf}
    \caption{Motivation for adopting bots and CAs.}
    \label{fig:motivations}
\end{figure}

%%%%%%%%%%%%%%%%%%%
\subsubsection{\underline{Code Bots}}
In this category, we group all the bots used to perform automatic operations on source code or related operations. We identified the sub-categories depicted following: 
%\gemma{parliamo di bot o di paper che parlano di bot? cioe nel senso forse è meglio scrivere che raggruppiamo i paper che usano i bot per ecc...che ne pensate?}\stefano{parliamo di bot perché per questa RQ volevamo estrarre le motivazioni di uso. Quindi abbiamo categorizzato le motivazioni in macro categorie. Una di queste sono i Code Bots. Forse potrei usare meno la parola bots e andare solo sulle motivazioni.}

\begin{description}[leftmargin=0.3cm]
    \item[Quality Bots.] This sub-category refers to bots that are used to (1) improve source code, (2) enhance quality by impacting product metrics, and (3) avoid and/or resolve technical debts. In our dataset, there are 13 formal studies~\citeA{carr2016automatic,paikari_2018_framework_chatbot_and_their_future,wyrich_2019_bot_for_code_refactoring,van_2019_programming_repair_bots,alizadeh_2019_refbot_software_refactoring_bot,hu_2019_improving_feedback_pull_request_with_bots,erlenhov_2020_bot_characteristics_and_challenges_from_practitioners,wessel_2020_code_review_bot_OSS,carvalho_2020_C_3PR_fix_static_analysis_violations,wyrich_2020_acceptance_of_refactoring_bots,wyrich_2021_bots_interaction_with_pull_requests,serban_2021_fixes_for_statyc_analysis_warning,sadi_2021_RAPID_bot_for_designing_web_APIs} and 4 grey studies~\citeB{best_bots_to_improve_your_software_development_process,storey2020_botse,four_Things_You_Absolutely_Need_to_Know_About_Software_Bots,software_bot_explained} ($\approx 22.07\%$ of the entire dataset).\\
    In particular, we found that most of the literature refers to \emph{Refactoring Bot}, i.e., used to perform refactoring operations on source code automatically~\citeA{wyrich_2019_bot_for_code_refactoring,alizadeh_2019_refbot_software_refactoring_bot,hu_2019_improving_feedback_pull_request_with_bots,carvalho_2020_C_3PR_fix_static_analysis_violations,wyrich_2020_acceptance_of_refactoring_bots,wyrich_2021_bots_interaction_with_pull_requests,serban_2021_fixes_for_statyc_analysis_warning}\citeB{best_bots_to_improve_your_software_development_process,four_Things_You_Absolutely_Need_to_Know_About_Software_Bots,software_bot_explained}. Then, some studies focus on using bots to enforce the application of formatting guidelines or requirements~\citeA{hu_2019_improving_feedback_pull_request_with_bots,sadi_2021_RAPID_bot_for_designing_web_APIs}\citeB{best_bots_to_improve_your_software_development_process} and good programming practices~\citeA{carr2016automatic}\citeB{best_bots_to_improve_your_software_development_process}. Finally, few of them report about \emph{Code Review Bots}, i.e., to automatize the code review process on pull requests (for example, on \textsc{GitHub})~\citeA{wessel_2020_code_review_bot_OSS}\citeB{storey2020_botse}.
    
    \item[Test Bots.] This sub-category refers to bots that support testers and similar figures during the testing activity. In our dataset, there are 10 formal studies~\citeA{wyrich_2020_acceptance_of_refactoring_bots,storey_2016_bot_uses_taxonomy,urli_2018_repairnator_project,paikari_2018_framework_chatbot_and_their_future,van_2019_programming_repair_bots,hu_2019_improving_feedback_pull_request_with_bots,monperrus_2019_automated_bug_fixes,khanan_2020_JITBot_just_in_time_defect_prediction_bot,erlenhov_2020_bot_characteristics_and_challenges_from_practitioners,erlenhov_2020_challenges_and_guidelines_for_test_bot_testing,okanovi_2020_chatbot_to_support_load_testing} ($\approx 12.98\%$ of the entire dataset).\\
    Most of the literature regards the use of bot for automation of test cases execution~\citeA{storey_2016_bot_uses_taxonomy,urli_2018_repairnator_project,van_2019_programming_repair_bots,hu_2019_improving_feedback_pull_request_with_bots,monperrus_2019_automated_bug_fixes,erlenhov_2020_challenges_and_guidelines_for_test_bot_testing,okanovi_2020_chatbot_to_support_load_testing}. Second, we found that many bots are used to identify bugs and perform automatic fixes~\citeA{storey_2016_bot_uses_taxonomy,urli_2018_repairnator_project,van_2019_programming_repair_bots,hu_2019_improving_feedback_pull_request_with_bots,monperrus_2019_automated_bug_fixes,wyrich_2020_acceptance_of_refactoring_bots}, \ie \emph{Repair Bot}, but also to detect possible implementation choices that could lead to defects in the code~\citeA{khanan_2020_JITBot_just_in_time_defect_prediction_bot}. Last, some works propose bots to (i) support developers in writing test code~\citeA{okanovi_2020_chatbot_to_support_load_testing} and (ii) implement heuristics to detect \emph{flaky tests}~\citeA{storey_2016_bot_uses_taxonomy}—i.e., tests exhibiting both a passing and failing behavior when run against the same code~\cite{luo2014_test_flakiness_definition}.
    
    \item[Configuration Bots.] This sub-category concerns to bots use to support practitioners during the setup and configuration processes of new software projects. In our dataset, there are 4 formal studies~\citeA{storey_2016_bot_uses_taxonomy,dey_2020_bot_that_commit_code,dey_2020_bot_commits,wyrich_2020_acceptance_of_refactoring_bots} and 1 grey study~\citeB{software_bot_explained} ($\approx 6.49\%$ of the entire dataset).\\
    From the identified literature, two works propose bots for automatically creating/modifying software configuration files or similar~\citeA{dey_2020_bot_that_commit_code,dey_2020_bot_commits}, while three works~\citeA{storey_2016_bot_uses_taxonomy,wyrich_2020_acceptance_of_refactoring_bots}\citeB{software_bot_explained} report about bots used to manage and monitor project dependencies.

    \item[CI/CD Bots.] This sub-category regards the usage of bots to support everyday activities in the context of CI/CD. In our dataset, 4 formal and 2 grey studies fit in this sub-category ($\approx 7.79\%$ of the entire dataset).\\
    Some studies analyze the usage of bots for monitoring software systems (for example, on \textsc{GitHub}) and performing automatic operations if certain conditions are met (e.g., automatically build the system on branch merge) ~\citeA{storey_2016_bot_uses_taxonomy,erlenhov_2020_bot_characteristics_and_challenges_from_practitioners}. Finally, five works study the use of bots to automatically trigger actions when specific criteria—related to no-code platforms—are met~\citeA{storey_2016_bot_uses_taxonomy,beschastnikh_2017_research_and_bot,wessel_2019_bot_close_abbandoned_pull_request_and_issues}\citeB{best_bots_to_improve_your_software_development_process,storey2020_botse}. For example, automatically creating an issue on GitHub when a bug is reported, or a task is assigned in the collaboration platform of the team (e.g., \textsl{Trello} and \textsl{Jira}). 
\end{description}

%%%%%%%%%%%%%%%%%%%
\subsubsection{\underline{Knowledge Bots}}

Under the category Knowledge Bots, we group all the bots use to share or manage information. In the following, we identify the sub-categories:

\begin{description}[leftmargin=0.3cm]
    \item[Information Bots.] This sub-category refers to the usage of bots for helping practitioners to manage and share valuable information related to specific projects and/or help complete implementation tasks. In our dataset, there are 12 formal studies~\citeA{storey_2016_bot_uses_taxonomy,tian2017APIbot,beschastnikh_2017_research_and_bot,paikari_2018_framework_chatbot_and_their_future,fukui_2019_bot_suggesting_questions,kumar_2019_sankie,ni_2019_CrowDevBot_CA_for_software_crowdsourcing,erlenhov_2020_bot_characteristics_and_challenges_from_practitioners,lin_2020_bot_framework_for_service_development_assistance,romero_2020_experiences_building_an_answer_bot,dominic_2020_bot_for_SE_newcomers,chatterjee_2021_automatic_extraction_of_opinion} and 4 grey studies~\citeB{best_bots_to_improve_your_software_development_process,storey2020_botse,bots_and_AI_in_project_management,bots_and_AI_in_project_management_2} that fit this sub-category ($\approx 20.77\%$ of the entire dataset).\\
    Most works propose bots to help practitioners answer questions or find documentation about a software module~\citeA{storey_2016_bot_uses_taxonomy,tian2017APIbot,fukui_2019_bot_suggesting_questions,romero_2020_experiences_building_an_answer_bot,dominic_2020_bot_for_SE_newcomers,chatterjee_2021_automatic_extraction_of_opinion}\citeB{storey2020_botse} (for example, find API documentation). Other studies are related to collecting and analyze product and process metrics, allowing practitioners to make aware decisions~\citeA{kumar_2019_sankie,lin_2020_bot_framework_for_service_development_assistance}\citeB{bots_and_AI_in_project_management,bots_and_AI_in_project_management_2}. Last, grey literature~\citeB{best_bots_to_improve_your_software_development_process,storey2020_botse} reports about the usage of bots to help onboarding new contributors for open-source projects: specifically, by providing knowledge to newcomers on how the community performs tasks and shares knowledge (e.g., templates for pull requests and guidelines for task boards).
    
    \item[Documentation Bots.] This sub-category regards bots used to help practitioners write and manage documenting artifacts related to their business processes and/or products. In our dataset, there are 8 formal studies~\citeA{storey_2016_bot_uses_taxonomy,paikari_2018_framework_chatbot_and_their_future,matthies_2019_bot_and_agile_retrospectives,perez_2019_CA_flexible_modelling,gilson_2019_NLP_and_collaborativeSE,dey_2020_bot_that_commit_code,dey_2020_bot_commits,ren_2020_collaborative_modelling_bot_vs_online_tools} and 1 grey study~\citeB{storey2020_botse} ($\approx 11.68\%$ of the entire dataset).\\
    Several works focus their attention on bots used to automatically create and update documenting artifacts~\citeA{gilson_2019_NLP_and_collaborativeSE,dey_2020_bot_that_commit_code,dey_2020_bot_commits}\citeB{storey2020_botse} (\eg code comments, documents, and reports). In particular, the state of the art~\citeA{storey_2016_bot_uses_taxonomy,ren_2020_collaborative_modelling_bot_vs_online_tools} has proposed bots to automatize the writing of notes for new software product releases, using NLP to synthesize developers' commit messages and comments. Other studies propose bots to improve and speed-up agile processes by automatizing the agile retrospective step by collecting metrics from different sources~\citeA{matthies_2019_bot_and_agile_retrospectives,ren_2020_collaborative_modelling_bot_vs_online_tools}. Last, bots are also used to record and document design decisions and, for some of them, generate static or behavioral models on-the-fly~\citeA{gilson_2019_NLP_and_collaborativeSE,ren_2020_collaborative_modelling_bot_vs_online_tools} (\eg UML graphs).
\end{description}

%%%%%%%%%%%%%%%%%%%
\subsubsection{\underline{Collaboration Bots}}

Under this category, we group all the bots used to improve and enhance communication, collaboration, and management activities. We identified the sub-categories in the following:

\begin{description}[leftmargin=0.3cm]
    \item[Management Bots.] This sub-category refers to bots used to help leading figures—\eg managers and team leaders—write artifacts and make decisions. In our dataset, there are 1 formal study~\citeA{basu_2021_bot_for_distribution_of_service_requests} and 2 grey studies~\citeB{bots_and_AI_in_project_management,bots_and_AI_in_project_management_2} that fit this sub-category ($\approx 3.89\%$ of the entire dataset).\\
    On the one side, some works use bot to assign people to the right task by using metrics and developers profiling~\citeA{basu_2021_bot_for_distribution_of_service_requests}\citeB{bots_and_AI_in_project_management}. On the other side, other studies predict and monitor risks at both project and business levels using bots~\citeB{bots_and_AI_in_project_management}, or collect performance data on team members~\citeB{bots_and_AI_in_project_management,bots_and_AI_in_project_management_2}.
    
        \item[Communication Bots.] This sub-category concerns bots used to help communication between practitioners. In our dataset, there are 9 formal studies~\citeA{storey_2016_bot_uses_taxonomy,paikari_2018_framework_chatbot_and_their_future,paikari_2019_chatbot_for_conflict_detection_and_resolution,gilson_2019_NLP_and_collaborativeSE,cerezo_2019_builing_an_expert_recommender_bot,erlenhov_2020_bot_characteristics_and_challenges_from_practitioners,mirsaeedi_2020_mitigating_turnover_with_bot,kim_2020_bot_to_facilitate_group_discussion,gilson_2020_recording_design_decision_on_the_fly} and 1 grey study~\citeB{storey2020_botse}($\approx 12.98\%$ of the entire dataset).\\
        Various works proposed ways to support information recording and sharing at CI/CD level: for example, by automatically (i) updating task status (on platforms like \textsl{Trello} and \textsl{Jira}) on commit and push action~\citeA{storey_2016_bot_uses_taxonomy} or (ii) detecting when two authors are working on the same file in order to reduce code conflicts~\citeA{paikari_2019_chatbot_for_conflict_detection_and_resolution}. Moreover, some of them report the possibility of using bots to collect metrics about a software artifact and provide—on-demand—information about the experts of such components~\citeA{cerezo_2019_builing_an_expert_recommender_bot,mirsaeedi_2020_mitigating_turnover_with_bot}. Furthermore, four works propose the usage of bots and conversational agents to support meeting activities by automatically recording and proposing old decisions—and associated rationale—when needed and requested~\citeA{gilson_2019_NLP_and_collaborativeSE,gilson_2020_recording_design_decision_on_the_fly}, or by moderating meetings by trying to allow all the participants to express their opinion equally~\citeA{kim_2020_bot_to_facilitate_group_discussion}\citeB{storey2020_botse}—for example, by implementing and supporting a round system for speaking. Last, related to knowledge sharing, a study proposes to use bot specifically to reduce \emph{turnover}—the phenomenon of continuous influx and retreat of human resources in a team~\cite{foucault2015_impact_of_turnover}—in an open-source software community by improving the reviewer selection process in code review~\citeA{mirsaeedi_2020_mitigating_turnover_with_bot}.

\end{description}

%%%%%%%%%%%%%%%%%%%
%\subsubsection{\underline{Other}}

%Under the category Other, we group all the bots that are used for very specific purposes and do not fall into any other categories. 


==> old/rq_2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/challenges.pdf}
    \caption{Bot Challenges Organization.}
    \label{fig:challenges}
\end{figure}

\subsection{RQ\textsubscript{2}: On the challenges of bots and conversational agents for software engineering purposes}

%\topar{Obiettivo della RQ e riassunto delle motivazioni}
The diffusion of bots and conversational agents for supporting software development processes has also led to the emergence of new challenges for computer scientists. 
For this reason, we investigated the challenges related to the interaction with, adoption, and development of bots for software engineering purposes.

Regarding the existing literature, Wessel et al.~\cite{wessel2021_dont_disturb_me_botChallenges} identified a series of challenges in the interactions with software bots in the open-source development context, with a particular focus on the concept of \emph{``noise''}---namely, annoying bot behaviors, \eg verbosity and unsolicited actions, which lead to deterioration of communication in teams. 
In terms of contributions, the authors provided a series of challenges experimented by practitioners, categorized under three main categories, \ie \textit{Interaction}, \textit{Adoption}, and \textit{Development Challenges}.

%\topar{Citare la figura e dire che di seguito si andranno a descrivere le principali categorie singolarmente}
On the one side, we found challenges already covered by Wessel et al.~\cite{wessel2021_dont_disturb_me_botChallenges}. On the other side, we contributed the state of the art with new challenges—indicated in Figure \ref{fig:challenges} with an orange box. 
Specifically, we decided to maintain the high-level separation proposed by Wessel et al.~\cite{wessel2021_dont_disturb_me_botChallenges}—the left side of Figure \ref{fig:challenges}—and to re-design the low-level categorization—the right side of the figure—based on the findings of our MLR.
The following subsections report in detail each identified challenge.

%\fabio{Dalla descrizione sopra, sembra che non abbiamo trovato niente di nuovo, il ché porterebbe un revisore a domandarsi del perché di questa RQ. E' davvero così? Vogliamo specificare che sì, teniamo la stessa high-level separation of concepts, ma includiamo nuove challenge estratte?}

%\fabio{Anche nelle successive sezioni relative alle challenge, non mi è chiaro cosa è nuovo e cosa era stato già trovato da Wessel. Potremmo essere più specifici. Vedo due modi: (1) Nella Figura 3, segnalare graficamente le nuove challenge identificate (con un asterisco, magari, o con un "new" da qualche parte); (2) Nel testo, eplicitare quali sono le challenge nuove e quali no.}
%%%%%%%%%%%%
\subsubsection{\underline{Interaction Challenges}}
\label{sec:interaction_challenges}

Most of the challenges identified by the literature regard the interaction between practitioners and bots. 
Such interaction can be intended as unidirectional—the user receives a message from the bot and reacts to it—and bidirectional—the user and the bot actively exchange messages.
%\topar{un poco di dati statistici, quanti paper parlano di questa categoria di challenge? 10 white e 4 grey}
In our dataset, there are 11 formal studies~\citeA{labeuf_2017_software_bots,srivastava_2019_architecture_applications_with_conversational_components,cerezo_2019_builing_an_expert_recommender_bot,pinheiro_2019_bot_development_challenges_motivations,castro_2019_bot_usability,melo_2020_what_do_devs_expect_from_CAs,erlenhov_2020_bot_characteristics_and_challenges_from_practitioners,abdellatif_2020_challenges_in_chatbot_development_from_stackoverflow,wyrich_2020_acceptance_of_refactoring_bots,wessel_2021_challenges_interacting_with_bot_on_OSS,saadat_2021_bots_modify_workflow_of_github_teams} and 5 grey studies~\citeB{storey2020_botse,bots_challenges_for_development,bots_challenges_for_development_2,bots_NLP_or_NLU,7_chatbot_development_challenges} that report on this challenge ($\approx 20.77\%$ of the entire dataset).

\begin{description}[leftmargin=0.3cm]
    \item[Interruption and Noise] One of the most reported challenges refers to the tendency of some bots to be unnecessarily verbose or useless~\citeA{labeuf_2017_software_bots,erlenhov_2020_bot_characteristics_and_challenges_from_practitioners,wessel_2021_challenges_interacting_with_bot_on_OSS,saadat_2021_bots_modify_workflow_of_github_teams}\citeB{storey2020_botse}. This behavior is defined by state of the art as \textbf{noise}, and it can significantly impact bot usage as well as communication and collaboration in the team. On the one side, bot design seems to represent the origin of this behavior —when the bot is intentionally designed to ``harass'' the developer. On the other side, a failure can lead bots to unexpected and noisy behaviors.
    
     \item[Communication.] Another challenge refers to the communication between the user and the bot~\citeA{srivastava_2019_architecture_applications_with_conversational_components,cerezo_2019_builing_an_expert_recommender_bot,pinheiro_2019_bot_development_challenges_motivations,lee_2019_accelerating_bots_development,castro_2019_bot_usability,melo_2020_what_do_devs_expect_from_CAs,erlenhov_2020_bot_characteristics_and_challenges_from_practitioners,abdellatif_2020_challenges_in_chatbot_development_from_stackoverflow,wyrich_2020_acceptance_of_refactoring_bots,wessel_2021_challenges_interacting_with_bot_on_OSS}\citeB{storey2020_botse,bots_challenges_for_development,bots_challenges_for_development_2,7_chatbot_development_challenges}. For example, \textbf{ensuring a short response time} comes to be mandatory for bot use: various bots—especially those based on API calls or off-the-shelf modules—are characterized by long responses to users' inputs and consequent frustration in them~\citeA{lee_2019_accelerating_bots_development}\citeB{bots_challenges_for_development_2}. Nevertheless, architectures of this type are often recommended for these software systems, and developers are faced with a trade-off between high modularity and maintainability—given by using such architectures—and fast response time.
     To continue, several works report the difficulty of bots in \textbf{providing practical and contextualized information}: indeed, bots should have information about the environment in which they are operating (\eg repositories address, commit template, and team composition), but this knowledge is difficult to collect automatically—and it is also related to privacy concerns~\citeA{melo_2020_what_do_devs_expect_from_CAs,wyrich_2020_acceptance_of_refactoring_bots,wessel_2021_challenges_interacting_with_bot_on_OSS}\citeB{storey2020_botse,bots_challenges_for_development_2}. Another primary concern regards how bots communicate with the user, specifically in the conversation design, generation of reply messages, and design of the chatbot's graphical user interface~\citeA{srivastava_2019_architecture_applications_with_conversational_components,cerezo_2019_builing_an_expert_recommender_bot,pinheiro_2019_bot_development_challenges_motivations,castro_2019_bot_usability,melo_2020_what_do_devs_expect_from_CAs,erlenhov_2020_bot_characteristics_and_challenges_from_practitioners,abdellatif_2020_challenges_in_chatbot_development_from_stackoverflow,wessel_2021_challenges_interacting_with_bot_on_OSS}\citeB{storey2020_botse,bots_challenges_for_development,7_chatbot_development_challenges}. Most practitioners struggle to \textbf{provide straightforward and satisfying user interfaces}, and researchers underline the \textbf{lack of guidelines and standards for bots usability}.

     \item[Natural Language Understanding and Processing] As already described in Section \ref{sec:background_related}, conversational agents' interactions are based and modeled on the concept of \emph{intent}, \ie a conceptual representation of a possible user request characterized by a set of mandatory information to fulfill the request (called \emph{entities}). Their correct interpretation is crucial for the bot operation and is often based on text interpretation using natural language processing (NLP) and understanding (NLU) algorithms. Therefore, \textbf{training NLP and NLU machine learning models} represented the most mentioned  challenge~\citeA{srivastava_2019_architecture_applications_with_conversational_components,cerezo_2019_builing_an_expert_recommender_bot,abdellatif_2020_challenges_in_chatbot_development_from_stackoverflow}\citeB{bots_NLP_or_NLU}; the main problem lies on the fact that a conversational agent works in singular contexts, and it is difficult to (1) extract sentences to train models and (2) reuse sentences from other contexts.

      \item[Ethical] Current literature also identified some challenges related to ethical aspects of bot operation~\citeA{cerezo_2019_builing_an_expert_recommender_bot,wessel_2021_challenges_interacting_with_bot_on_OSS}\citeB{storey2020_botse}. 
     For example, practitioners tend to be \textbf{skeptical because of past experiences with bots exposing malicious intents}—\eg theft of sensitive information or insertion of malicious code. So, interacting with these bots can be challenging because their identification is not always an easy task~\citeA{wessel_2021_challenges_interacting_with_bot_on_OSS}.
    In addition, another challenge is related to a well-known topic such \emph{fairness}~\cite{verma2018_fairness_definition}, intended as the equitable and just treatment—without discrimination—assumed by software systems—particularly in the context of artificial intelligence. Specifically, conversational agents are based on trained machine learning models using datasets containing sentences and assertions by potential users, thus possibly leading the bot to be biased given the different culture and background of the individuals who built the dataset, which could \textbf{lead to unexpected and often discriminatory behaviors}~\citeA{wessel_2021_challenges_interacting_with_bot_on_OSS}.
    Last but not least, the literature highlighted the phenomena known as \emph{Uncanny Valley}—i.e., the phenomenon whereby a computer behaving like a human being evokes a sense of unease and revulsion in the person interacting with it~\cite{mori2012_uncanny_valley, kageki2012_uncanny_valley}. The phenomenon is extremely diffused, especially in the interaction with conversational agents. It is related to the humanization of robots: people tend to exhibit unpleasant feelings—such as revulsion and uneasiness comparable to perturbation—when interacting with machines with overly ``human'' attitudes. Managing this phenomenon so that \textbf{the bots turn out to be human enough to improve communication without being disturbing} is a difficult challenge~\citeA{cerezo_2019_builing_an_expert_recommender_bot,wessel_2021_challenges_interacting_with_bot_on_OSS}\citeB{storey2020_botse}.
\end{description}

%\topar{Interruption and Noise descrizione}
%One of the most reported challenges in such a category regards the tendency of some bots to be unnecessarily verbose or useless~\citeA{labeuf_2017_software_bots,erlenhov_2020_bot_characteristics_and_challenges_from_practitioners,wessel_2021_challenges_interacting_with_bot_on_OSS}\citeB{storey2020_botse}. The result of such behavior is defined by state of the art as \textbf{noise}, and it can significantly impact bot usage as well as communication and collaboration in the team. The literature identified the origin of such behavior in bot design—when the bot is intentionally designed to ``harass'' developers—or by failures that lead bots to unexpected and noisy behaviors.

%\topar{Communication descrizione}
%Another challenge our survey identified is related to the communication between the user and the bot~\citeA{srivastava_2019_architecture_applications_with_conversational_components,cerezo_2019_builing_an_expert_recommender_bot,pinheiro_2019_bot_development_challenges_motivations,lee_2019_accelerating_bots_development,castro_2019_bot_usability,melo_2020_what_do_devs_expect_from_CAs,erlenhov_2020_bot_characteristics_and_challenges_from_practitioners,abdellatif_2020_challenges_in_chatbot_development_from_stackoverflow,wyrich_2020_acceptance_of_refactoring_bots,wessel_2021_challenges_interacting_with_bot_on_OSS}\citeB{storey2020_botse,bots_challenges_for_development,bots_challenges_for_development_2}. For example, \textbf{ensuring a short response time} comes to be mandatory for bot use: various bots—especially those based on API calls or off-the-shelf modules—are characterized by long responses to users' inputs and consequent frustration in them~\citeA{lee_2019_accelerating_bots_development}\citeB{bots_challenges_for_development_2}. Nevertheless, architectures of this type are often recommended for these software systems, and developers are faced with a choice between using them—which provides greater maintainability—and faster response times.
%Furthermore, several works report on the difficulty of bots in \textbf{providing practical and contextualized information}: to do so, bots should have information about the environment in which they are operating (\eg repositories address, commit template, and team composition), but such knowledge is difficult to collect automatically—and it is also related to privacy concerns~\citeA{melo_2020_what_do_devs_expect_from_CAs,wyrich_2020_acceptance_of_refactoring_bots,wessel_2021_challenges_interacting_with_bot_on_OSS}\citeB{storey2020_botse,bots_challenges_for_development_2}.
%Another primary concern regards how bots communicate with the user, specifically in the conversation design, generation of reply messages, and design of the chatbot's graphical user interface~\citeA{srivastava_2019_architecture_applications_with_conversational_components,cerezo_2019_builing_an_expert_recommender_bot,pinheiro_2019_bot_development_challenges_motivations,castro_2019_bot_usability,melo_2020_what_do_devs_expect_from_CAs,erlenhov_2020_bot_characteristics_and_challenges_from_practitioners,abdellatif_2020_challenges_in_chatbot_development_from_stackoverflow,wessel_2021_challenges_interacting_with_bot_on_OSS}\citeB{storey2020_botse,bots_challenges_for_development}. Most practitioners struggle to \textbf{provide straightforward and satisfying user interfaces}, and researchers underline the \textbf{lack of guidelines and standards for bots usability}.

%\topar{NLP and NLU challenges description}
%As already described in Section \ref{sec:background_related}, conversational agents' interactions are on the concept of \emph{intent}, \ie a conceptual representation of a possible user request to the bot characterized by a set of information mandatory to fulfill the request (called \emph{entities}). The correct interpretation of such intents is fundamental for the bot operation and is often based on text interpretation using natural language processing (NLP) and understanding (NLU) algorithms. Therefore, \textbf{training such NLP and NLU machine learning models} is a highly reported challenge~\citeA{srivastava_2019_architecture_applications_with_conversational_components,cerezo_2019_builing_an_expert_recommender_bot,abdellatif_2020_challenges_in_chatbot_development_from_stackoverflow}\citeB{bots_NLP_or_NLU}; the main difficulty lies in the fact that a conversational agent works in particular contexts, and it is difficult to (1) extract sentences to train models and (2) reuse sentences from other contexts.

%\topar{Ethical challenges description}
%State of the art also identified some challenges related to the ethical aspect of bot operation~\citeA{cerezo_2019_builing_an_expert_recommender_bot,wessel_2021_challenges_interacting_with_bot_on_OSS}\citeB{storey2020_botse}. 
%For example, practitioners \textbf{tend to be skeptical of cause past experiences with bots exposing malicious intents}—\eg theft of sensitive information or insertion of malicious code. Interacting with such types of bots can be challenging because their identification is not always an easy task~\citeA{wessel_2021_challenges_interacting_with_bot_on_OSS}.
%In addition, an ulterior challenge is related to the well-known topic of \emph{fairness}~\cite{verma2018_fairness_definition}, intended as the equitable and just treatment—without discrimination—assumed by software systems—particularly in the context of artificial intelligence. Specifically, conversational agents are based on machine learning models that are trained using datasets containing sentences and assertions by potential users. As for other machine learning fields, also this is subject to bias caused by the culture and background of the individuals who built the dataset, which could \textbf{lead to unexpected and often discriminatory behaviors}~\citeA{wessel_2021_challenges_interacting_with_bot_on_OSS}.
%Last but not least, the literature identified the phenomena known as \emph{Uncanny Valley}—i.e., the phenomenon whereby a computer behaving like a human being evokes a sense of unease and revulsion in the person interacting with it~\cite{mori2012_uncanny_valley, kageki2012_uncanny_valley}—as extremely diffused, specifically in the interaction with conversational agents. Such a phenomenon is related to the humanization of robots: people tend to exhibit unpleasant feelings—such as revulsion and uneasiness comparable to perturbation—when interacting with machines with overly ``human'' attitudes. Managing this phenomenon so that \textbf{the bots turn out to be human enough to improve communication without being disturbing} is a difficult challenge~\citeA{cerezo_2019_builing_an_expert_recommender_bot,wessel_2021_challenges_interacting_with_bot_on_OSS}\citeB{storey2020_botse}.

%%%%%%%%%%%%
\subsubsection{\underline{Adoption Challenges}}
\label{sec:adoption_challenges}

%\todo[inline]{\stefano{Da riscrivere perché secondo me è assai bruttina}}

Several studies reported challenges in adopting bots and chatbots for development reasons. 
In our dataset, there are 8 formal studies~\citeA{storey_2016_bot_uses_taxonomy,van_2019_programming_repair_bots,monperrus_2019_automated_bug_fixes,brown_2019_bots_for_effective_recommendations,erlenhov_2020_bot_characteristics_and_challenges_from_practitioners,brown_2020_recommendation_for_bot_architectures,wyrich_2021_bots_interaction_with_pull_requests,wessel_2021_challenges_interacting_with_bot_on_OSS} and 3 grey studies~\citeB{storey2020_botse,software_bot_explained,7_chatbot_development_challenges} that report on such a category ($\approx 14.28\%$ of the entire dataset).

\begin{description}[leftmargin=0.3cm]
    \item[Motivation and Trust] According to various studies, the first challenge involves \textbf{motivating practitioners to use bots}~\citeA{monperrus_2019_automated_bug_fixes,erlenhov_2020_bot_characteristics_and_challenges_from_practitioners,wessel_2021_challenges_interacting_with_bot_on_OSS}\citeB{storey2020_botse,software_bot_explained,7_chatbot_development_challenges}. In fact, various practitioners are skeptical of bots because of bias—they think they can implement malicious behaviors or are useless and noisy, underlining a \textbf{lack of trust}~\citeA{monperrus_2019_automated_bug_fixes,brown_2019_bots_for_effective_recommendations,erlenhov_2020_bot_characteristics_and_challenges_from_practitioners,brown_2020_recommendation_for_bot_architectures,wyrich_2021_bots_interaction_with_pull_requests}\citeB{storey2020_botse,software_bot_explained,7_chatbot_development_challenges} of developers in bots' recommendations.

    \item[Discoverability and Customization] Furthermore, \textbf{identifying the correct bot to solve a problem is challenging}~\citeA{storey_2016_bot_uses_taxonomy,wessel_2021_challenges_interacting_with_bot_on_OSS} for two reasons: first, there are limited search mechanisms to identify appropriate bots given a problem; second, the lack of a unified standard to characterize bots leads to difficulties in their description and categorization.
    This becomes even more problematic when practitioners identify the correct bot but have \textbf{difficulty configuring it}~\citeA{van_2019_programming_repair_bots,wessel_2021_challenges_interacting_with_bot_on_OSS}. In fact, such systems often have few configuration options, even if they have to be used in significantly different contexts.
\end{description}

%%%%%%%%%%%%
\subsubsection{\underline{Development Challenges}}
\label{sec:development_challenges}

Last, we identified several challenges related to the development of bots. 
In our dataset, there are 9 formal studies~\citeA{zamanirad2017programming,srivastava_2019_architecture_applications_with_conversational_components,pinheiro_2019_bot_development_challenges_motivations,abdellatif_2020_challenges_in_chatbot_development_from_stackoverflow,brown_2020_recommendation_for_bot_architectures,erlenhov_2020_challenges_and_guidelines_for_test_bot_testing,perez_2021_creating_and_migrating_chatbot,cabot_2021_testing_challenges_for_NLP_intensive_bots,wessel_2021_challenges_interacting_with_bot_on_OSS} and 6 grey studies~\citeB{bots_challenges_for_development_2,10_best_chatbot_framework,top_framework_part_1,probot,8_chatbot_environments,understanding_CA_architecture} that report on such a category ($\approx 19.48\%$ of the entire dataset).

\begin{description}[leftmargin=0.3cm]
    \item[Framework, Architecture, and Integration] First of all, various actors have proposed various frameworks to support developers in the development of bots and chatbots (\eg Microsoft Azure Bot Framework, Google DialogFlow, Amazon Lex, and Rasa). Although such variety can provide practitioners with a large plethora of possibilities to reach their objectives, the literature identifies a \textbf{difficulty in identifying the correct framework to start development}~\citeA{pinheiro_2019_bot_development_challenges_motivations,abdellatif_2020_challenges_in_chatbot_development_from_stackoverflow,perez_2021_creating_and_migrating_chatbot,wessel_2021_challenges_interacting_with_bot_on_OSS}\citeB{10_best_chatbot_framework,top_framework_part_1,probot,8_chatbot_environments}. Such a challenge arises for three main reasons. First, the enormous plethora of frameworks that implement the same functionalities makes it hard to select the better one. Second, the lack of readable documentation for each framework ulteriorly hardens the decision process. Third, \textbf{bots are complex systems to design from an architectural point of view}~\citeA{srivastava_2019_architecture_applications_with_conversational_components,brown_2020_recommendation_for_bot_architectures}\citeB{understanding_CA_architecture} because, to improve modularity, engineers push to adopt client-server architectures in which the core functionalities are implemented on the server and the interaction with the user on the client side. This, in addition to adding complexity due to the management of communication protocols between the various components (\eg HTTPS, API Call, and Service Calls), often makes it necessary to use different technologies for the same system, and \textbf{not all bot frameworks allow easy integration with them}~\citeA{pinheiro_2019_bot_development_challenges_motivations,abdellatif_2020_challenges_in_chatbot_development_from_stackoverflow}.

    \item[Testing] Furthermore, despite such a large amount of frameworks, \textbf{a significant minority support developers in testing activities of bots and CAs}~\citeA{srivastava_2019_architecture_applications_with_conversational_components,pinheiro_2019_bot_development_challenges_motivations,erlenhov_2020_challenges_and_guidelines_for_test_bot_testing,cabot_2021_testing_challenges_for_NLP_intensive_bots}\citeB{bots_challenges_for_development_2}. This is a significant problem because the lack of testing for such a system contributes to the mistrust of practitioners when they have to use them. Underlying this lack is the difficulty in automating the interactions between a human user and the bot. Furthermore, the large number of frameworks for bot development makes it difficult to provide a single tool capable of testing for all.

    \item[Maintenance] Such a challenge in terms of testing leads to the emergence of another one: \textbf{the maintenance—and consequent evolution—of bots is challenging}~\citeA{zamanirad2017programming,erlenhov_2020_challenges_and_guidelines_for_test_bot_testing,wessel_2021_challenges_interacting_with_bot_on_OSS}. In fact, the lack of tests and the difficulty in monitoring such systems can impact maintenance activities, making it hard to identify and fix a bug.
\end{description}


==> sd.tex <==
\begin{table}
    \centering
    \caption{Identified Best Practices for \textbf{Bots Interaction and Adoption}.}
    \vspace{1mm} % Adjust the height of the space between caption and tabular
    
    \rowcolors{1}{graytable}{white}
    \resizebox{\linewidth}{!}{
\begin{tabular}{lrlrrllllrlrlllllll}
\rowcolor[HTML]{000000} 
{\color[HTML]{FFFFFF} }                                                                                                          & {\color[HTML]{FFFFFF} \textbf{Interruption and Noise}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Long Response Latency}}} & {\color[HTML]{FFFFFF} \textbf{Contextual Information}} & {\color[HTML]{FFFFFF} \textbf{Usability}}    & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{NLP and NLU}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Uncanny Valley}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Malicious Intent}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Bias Information}}} & {\color[HTML]{FFFFFF} \textbf{Motivation}}   & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Discoverability}}} & {\color[HTML]{FFFFFF} \textbf{Trust}}        & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Terms of Serveice}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Configuration and Customization}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Framework}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Testing}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Maintenance}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Architecture}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Integration}}} \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Implement a System to evaluate bot choices}}                               & 1                                                      &                                                                                                   & 1                                                      & 1                                            &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                              &                                                                                              &                                                                                              & 1                                            &                                                                                             & 1                                            &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                            &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Follow a modular architecture}}                                            & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                                     & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           & 1                                            & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                           &                                                                                            &                                                                                              &                                                                                              & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                             & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                               &                                                                                                             &                                                                                       & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                       & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                           & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}2}                                            &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Make bots adaptive and able to learn over time using AI}}                  & 1                                                      & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                                     & 2                                                      & 2                                            &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                              &                                                                                              &                                                                                              & 1                                            &                                                                                             & 2                                            &                                                                                               &                                                                                                             &                                                                                       & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                       &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}2}                                            &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Adopt a specific lifecycle process for bots}}                              & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           &                                                                                                   & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                         &                                                                                            &                                                                                              &                                                                                              & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                             & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         &                                                                                          &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Carefully select the correct framework based on bot requirements}}         & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           &                                                                                                   & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                         &                                                                                            &                                                                                              &                                                                                              & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                             & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                               &                                                                                                             & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}4}                                         &                                                                                     &                                                                                         &                                                                                          &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Integrate bots actions in a way that do not interrupt developer workflow}} & 1                                                      &                                                                                                   & 1                                                      & 2                                            &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                              &                                                                                              &                                                                                              & 2                                            &                                                                                             & 3                                            &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         &                                                                                          &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Allow developers to edit bot configuration easily}}                        & 1                                                      &                                                                                                   & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           & 1                                            & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                           &                                                                                            &                                                                                              &                                                                                              & 1                                            &                                                                                             & 1                                            &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         &                                                                                          &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Provide bot with personality}}                                             & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           &                                                                                                   & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           & 1                                            &                                                                                         &                                                                                            &                                                                                              &                                                                                              & 1                                            &                                                                                             & 1                                            &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         &                                                                                          &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Design a Smooth and frictionless interaction}}                             & 2                                                      &                                                                                                   & 2                                                      & 2                                            &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                              &                                                                                              &                                                                                              & 1                                            &                                                                                             & 2                                            &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         &                                                                                          &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Enforce transparency in bot actions and outputs}}                          & 2                                                      &                                                                                                   & 1                                                      & 1                                            &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                              &                                                                                              &                                                                                              & 2                                            &                                                                                             & 2                                            &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         &                                                                                          &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Integrating concepts from behavioral science in interaction flow}}         & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           &                                                                                                   & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                         &                                                                                            &                                                                                              &                                                                                              & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                             & 1                                            &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                            &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Provide users with a high level of control over bot}}                      & 2                                                      &                                                                                                   & 3                                                      & 3                                            &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                              &                                                                                              &                                                                                              & 2                                            &                                                                                             & 3                                            &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         &                                                                                          &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Create a reliable test infrastructure}}                                    & 1                                                      & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                                     & 1                                                      & 1                                            &                                                                                         &                                                                                            &                                                                                              &                                                                                              & 1                                            &                                                                                             & 1                                            &                                                                                               &                                                                                                             &                                                                                       & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                       &                                                                                         &                                                                                          &                                                                                        
\end{tabular}
}
    
    \label{table:best_practices_interaction}
\end{table}

==> sections/old_methodology.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Research Objectives and Questions}

\tostruct{Obiettivi}

\tostruct{Research questions}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Motivations for Conducting a MLR}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Research Query Definition}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Search Databases}

\subsubsection{Formal Literature}

\subsubsection{Grey Literature}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Exclusion and Inclusion Criteria}

\subsubsection{Formal Literature}

\subsubsection{Grey Literature}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Quality Assessment}

\subsubsection{Formal Literature}

\subsubsection{Grey Literature}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Data Extraction}

==> sections/old_table_discussion.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
%\begin{landscape}
\begin{table}[]
\centering
\caption{Match between best practices and challenges - Part 1. \stefano{consapevole del fatto che so brutte, se le lasciamo le modifico}}
\vspace{1mm} % Adjust the height of the space between caption and tabular

\resizebox{\linewidth}{!}{%
\begin{tabular}{|
>{\columncolor[HTML]{000000}}p{0.3\linewidth} |
>{\columncolor[HTML]{FFFFFF}}r 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}r 
>{\columncolor[HTML]{FFFFFF}}r 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l |}
\toprule
\multicolumn{1}{|c|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} }} &
  \multicolumn{8}{c|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Challenges - Part 1}}} \\ \cline{2-9} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Best Practices}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Interruption and Noise}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Long Response Latency}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Contextual Information}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Usability}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{NLP and NLU}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Uncanny Valley}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Malicious Intent}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Bias Information}}}} \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Implement a System to evaluate bot choices}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Follow a modular architecture}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Make bots adaptive and able to learn over time using AI}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Adopt a specific lifecycle process for bots}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Carefully select the correct framework based on bot requirements}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Integrate bots actions in a way that do not interrupt developer workflow}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Allow developers to edit bot configuration easily}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Provide bot with personality}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Design a Smooth and frictionless interaction}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Enforce transparency in bot actions and outputs}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Integrating concepts from behavioral science in interaction flow}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Provide users with a high level of control over bot}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}3} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Create a reliable test infrastructure}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
   \bottomrule
\end{tabular}%
}
\label{table:cahllenge_best_practices_1}
\end{table}

\begin{table}[]
    \centering
\caption{Match between best practices and challenges - Part 2.}
\vspace{1mm} % Adjust the height of the space between caption and tabular

\resizebox{\linewidth}{!}{%
    \begin{tabular}{|
>{\columncolor[HTML]{000000}}p{0.3\linewidth} |
>{\columncolor[HTML]{FFFFFF}}r 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}r 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l |}
\toprule
\multicolumn{1}{|c|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} }} &
  \multicolumn{10}{c|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Challenges - Part 2}}} \\ \cline{2-11} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Best Practices}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Motivation}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Discoverability}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Trust}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Terms of Serveice}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Configuration and Customization}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Framework}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Testing}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Maintenance}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Architecture}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Integration}}}} \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Implement a System to evaluate bot choices}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Follow a modular architecture}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Make bots adaptive and able to learn over time using AI}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Adopt a specific lifecycle process for bots}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Carefully select the correct framework based on bot requirements}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}4} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Integrate bots actions in a way that do not interrupt developer workflow}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Allow developers to edit bot configuration easily}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Provide bot with personality}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Design a Smooth and frictionless interaction}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Enforce transparency in bot actions and outputs}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Integrating concepts from behavioral science in interaction flow}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Provide users with a high level of control over bot}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Create a reliable test infrastructure}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
   \bottomrule
\end{tabular}%
}
    \label{table:cahllenge_best_practices_2}
\end{table}

